Statistical Parameterized Physics-Based Machine Learning Digital Twin Models for Laser Powder Bed Fusion Process

A digital twin (DT) is a virtual representation of physical process, products and/or systems that requires a high-fidelity computational model for continuous update through the integration of sensor data and user input. In the context of laser powder bed fusion (LPBF) additive manufacturing, a digital twin of the manufacturing process can offer predictions for the produced parts, diagnostics for manufacturing defects, as well as control capabilities. This paper introduces a parameterized physics-based digital twin (PPB-DT) for the statistical predictions of LPBF metal additive manufacturing process. We accomplish this by creating a high-fidelity computational model that accurately represents the melt pool phenomena and subsequently calibrating and validating it through controlled experiments. In PPB-DT, a mechanistic reduced-order method-driven stochastic calibration process is introduced, which enables the statistical predictions of the melt pool geometries and the identification of defects such as lack-of-fusion porosity and surface roughness, specifically for diagnostic applications. Leveraging data derived from this physics-based model and experiments, we have trained a machine learning-based digital twin (PPB-ML-DT) model for predicting, monitoring, and controlling melt pool geometries. These proposed digital twin models can be employed for predictions, control, optimization, and quality assurance within the LPBF process, ultimately expediting product development and certification in LPBF-based metal additive manufacturing.

==> table1.tex <==
\begin{table}[t!]
\vspace{-1mm}
\centering
\scalebox{0.8}{
\begin{tabular}{c|cc|cc|cc}
\toprule
\multirow{2}{*}{Method}              & \multicolumn{2}{c|}{\textbf{UT-Zappos50K}} & \multicolumn{2}{c|}{\textbf{Wider Attribute}} & \multicolumn{2}{c}{\textbf{CUB-200-2011}} \\
                                     & Top-1 Acc.              & Top-5 Acc.              & Top-1 Acc.            & Top-5 Acc.            & Top-1 Acc.               & Top-5 Acc.               \\ \midrule \midrule \multicolumn{7}{c}{\it (Supervised) Labels + Cl-InfoNCE} \\ \midrule
SupCon~\citep{khosla2020supervised}      & 89.0$\pm$0.4                & 99.4$\pm$ 0.3              & 49.9$\pm$0.8             & 76.2$\pm$0.2             & 59.9$\pm$0.7                & 78.8$\pm$ 0.3               \\ \midrule \midrule \multicolumn{7}{c}{\it   (Weakly-supervised) Attributes-Determined Clusters + Cl-InfoNCE} \\ \midrule
Ours      & 84.6$\pm$0.4                & 99.1$\pm$0.2               & 45.5$\pm$0.2            & 75.4$\pm$0.2             & 20.6$\pm$ 0.5               & 47.0$\pm$0.5                \\
%\midrule \midrule \multicolumn{7}{c}{\it Self-supervised Representation Learning (clustering-based, $Z=$ unsupervised clusters)} \\ \midrule \midrule
%$^\ddagger$SwAV~\citep{caron2020unsupervised}   & xxx$\pm$xxx                & xxx$\pm$xxx               & xxx$\pm$xxx             & xxx$\pm$xxx             & xxx$\pm$xxx               & xxx$\pm$xxx   \\ [1mm]
%$^\dagger$PCL~\citep{li2020prototypical} & 82.4$\pm$0.5               & xxx$\pm$xxx               & 41.0$\pm$0.4             & xxx$\pm$xxx             & 14.4$\pm$0.5               & xxx$\pm$xxx                \\[1mm]
%$^\dagger$K-means Clusters + Cl-InfoNCE (ours)     & 84.5$\pm$0.4                & xxx$\pm$xxx               & 43.6$\pm$0.4         & xxx$\pm$xxx             & 17.6$\pm$0.2               & xxx$\pm$xxx \\
 %\midrule \midrule \multicolumn{7}{c}{\it Self-supervised Representation Learning (non-clustering-based, $Z=$ instance id)} \\
  \midrule \midrule \multicolumn{7}{c}{\it  (Self-supervised) Instance-ID + Cl-InfoNCE} \\
 \midrule
    SimCLR~\citep{chen2020simple} & 77.8$\pm$1.5                & 97.9$\pm$0.8               & 40.2$\pm$0.9             & 73.0$\pm$0.3             & 14.1$\pm$ 0.7               & 35.2$\pm$0.6            \\\bottomrule
\end{tabular}
}
\vspace{-1mm}
\caption{\small Experimental results for different supervision levels with the presented Cl-InfoNCE objective.
%under supervised (pre-training using label supervision), weakly supervised (pre-training using data attributes), and conventional self-supervised (pre-training using neither label supervision nor data attributes) setting.
%Except for the CMC approach, each setting refers to a particular cluster construction  ($Z = $  downstream labels, attributes-determined clusters, and instance ID).
%The methods presented in this table are either contrastive or predictive learning approaches.
For weakly-supervised methods that consider attributes-determined clusters, we report the best results by tuning the hyper-parameter $k$. The results suggest that, with the help of auxiliary information, we can better close the performance gap between supervised and self-supervised representations.
}
\label{tbl:attributes-supervision}
\vspace{-4mm}
\end{table}
